Large Investment Model

Traditional quantitative investment research is encountering diminishing returns alongside rising labor and time costs. To overcome these challenges, we introduce the Large Investment Model (LIM), a novel research paradigm designed to enhance both performance and efficiency at scale. LIM employs end-to-end learning and universal modeling to create an upstream foundation model capable of autonomously learning comprehensive signal patterns from diverse financial data spanning multiple exchanges, instruments, and frequencies. These "global patterns" are subsequently transferred to downstream strategy modeling, optimizing performance for specific tasks. We detail the system architecture design of LIM, address the technical challenges inherent in this approach, and outline potential directions for future research. The advantages of LIM are demonstrated through a series of numerical experiments on cross-instrument prediction for commodity futures trading, leveraging insights from stock markets.

==> authorbio.tex <==
\clearpage
\addcontentsline{toc}{section}{Author Biographies}
\section*{Author Biographies}
  \begin{wrapfigure}{l}{25mm} 
    \includegraphics[width=1.1in,height=1.5in,clip,keepaspectratio]{thumbnails/JianGuo2.png}
  \end{wrapfigure}\par
  \textbf{Jian Guo} is currently the Executive President and a Chief Scientist at International Digital Economy Academy (IDEA). Dr. Guo also serves as an Adjunct Professor of Artificial Intelligence at The Hong Kong University of Science and Technology (Guangzhou), an Affiliated Professor of Shanghai Advanced Institute of Finance (SAIF) at Shanghai Jiao Tong University and a Professor of Practice at Tsinghua University. Dr. Guo received his B.S. in mathematics from Tsinghua University, and received his Ph.D. in statistics from University of Michigan. He started his professorship (tenure-track) at Harvard University since 2011. Dr. Guo is one of the pioneering AI finance researchers, and is an entrepreneur in quantitative investment industry.\par

~\\

\newpage
\section*{}
  \begin{wrapfigure}{l}{25mm} 
    \includegraphics[width=1.1in,height=1.5in,clip,keepaspectratio]{thumbnails/harryShum1.png}
  \end{wrapfigure}\par
  \textbf{Heung-Yeung Shum} is the Founding Chairman of International Digital Economy Academy (IDEA), and the Council Chairman of The Hong Kong University of Science and Technology. He is a Foreign Member of National Academy of Engineering of the US, International Fellow of Royal Academy of Engineering of the UK, ACM Fellow and IEEE Fellow. Until March 2020, he was the Executive Vice President of Microsoft Corporation, responsible for AI and Research. Dr. Shum received his Ph.D. in Robotics from School of Computer Science at Carnegie Mellon University. \par



==> introduction.tex <==
 
\section{Quant4.0+: Rethinking AI Investment}
Quantitative investment (quant) involves financial investment strategies driven by mathematical, statistical, or machine learning models. Powerful computers execute trading instructions derived from quant models at speeds and frequencies unattainable by human traders. As discussed in the Quant4.0 article~\cite{guo2022quant}, the rise of artificial intelligence is reshaping the paradigm of quantitative investment. The rapid advancement of artificial general intelligence (AGI) and multi-modal large language models (LLMs) \cite{yin2024survey} in the past two years inspires a reconsideration of the future trajectory of quantitative investment technology. The success of GPT-like models \cite{brown2020language,openai2024gpt4} has demonstrated the immense value of end-to-end deep neural network modeling and generative AI using self-supervised learning \cite{balestriero2023cookbook}, which can influence quantitative investment technology in at least three key areas:
\begin{enumerate}[noitemsep,topsep=0pt] 
    \item Many examples in natural language processing \cite{zhou_neuralNLP_2020} and computer vision \cite{li2023multimodal} have demonstrated that, with ample data, end-to-end modeling with large-scale deep learning has great opportunity to outperform traditional machine learning models and statistical analytics pipelines. This necessitates re-evaluating the traditional quantitative research pipeline, especially the role of financial factors in quantitative strategy development. For high-frequency trading~\cite{Beckhardt_hifreq2016}, the abundance of trading records can support deep learning models' end-to-end training without explicit feature engineering (like financial factor construction). This enables models to be trained directly on original data, outputting alphas, positions, or even executable orders. Conversely, in low-frequency investment approaches such as fundamental or event-driven investing \cite{tulchinsky2015finding}, the sparsity of samples limits straightforward end-to-end learning. In this scenarios, large language models can be instrumental in end-to-end prediction. For instance, LLMs can analyze financial news, financial statements, analyst reports, corporate announcements, and various other textual (or multi-modal) information to generate investment decision signals or alphas directly, bypassing the conventional step of textual factor mining with task-specific NLP models (e.g., sentiment prediction models \cite{Wnkhade_2022}, opinion mining models \cite{Koufakou_2023}).
    \item Large foundational models pre-trained on vast datasets demonstrate substantial generalizability and scalability. Proper fine-tuning \cite{han2024parameterefficient} tailored to specific tasks significantly enhances their predictive capabilities, often outperforming those models that are specialized for those tasks. This raises the question: is the "pre-trained foundational models + fine-tuned specialized models" paradigm suitable for quantitative strategy research? Traditionally, quantitative hedge funds have invested considerable labor and time in researching numerous "small" models to trade various financial instruments across different markets and strategies. If a robust foundational model \cite{zhou2023comprehensive} for quantitative investment can uncover transferable trading patterns and investment logic across various instruments and markets, quantitative strategy research could become a fine-tuning task for specific strategy demands and investment scenarios, vastly improving research efficiency.
    \item The transformative power of multi-modal large language models is rapidly advancing fundamental investing by integrating vast and varied alternative data sources. Pre-processing, analyzing, and modeling alternative data to extract new-dimensional alphas has traditionally been considered laborious and inefficient "dirty work" by most trading firms, due to the sheer volume, diversity, and unstructured nature of the data. However, the advent of LLMs offers significant breakthroughs in overcoming these challenges.
\end{enumerate}

Given these considerations, we introduce a new quant research paradigm, Quant4.0+, which reinterprets the three key components of Quant4.0 with the state-of-the-art end-to-end modeling and pre-trained foundation model for quantitative investment. On one hand, end-to-end modeling provides a more efficient and convenient technical route for automated AI in Quant4.0, compared to autoML-related techniques \cite{HE2021106622} that use automated search to find optimal solutions for each step in the quant pipeline. On the other hand, LLMs' powerful reasoning ability makes them excellent "interpreters" for explainable AI and "analysts" for knowledge-driven AI in Quant4.0.

The rest of this article is organized as follows. Section~\ref{sec_datadiversity} introduces the characteristics of diverse data in quantitative trading. Section~\ref{sec_e2e_quant} introduces three types of end-to-end modeling paradigms derived from the traditional quant research pipeline. Section~\ref{sec_LIM} explains how large investment models can enhance end-to-end modeling by utilizing diverse global data to pre-train an upstream foundational model for downstream quant modeling tasks. Section~\ref{sec_research_directions} lists a number of research directions to further improve LIM. Section~\ref{sec_related_work} reviews existing research related to end-to-end quant modeling and LLM-based investing. Section~\ref{sec_conclusion} summarizes the difference between Quant4.0 and Quant4.0+, and forecasts the future development trends.
